Hyperparameter Optimization: Foundations, Algorithms, Best Practices and Open Challenges

Most machine learning algorithms are configured by one or several hyperparameters that must be carefully chosen and often considerably impact performance. To avoid a time consuming and unreproducible manual trial-and-error process to find well-performing hyperparameter configurations, various automatic hyperparameter optimization (HPO) methods, e.g., based on resampling error estimation for supervised machine learning, can be employed. After introducing HPO from a general perspective, this paper reviews important HPO methods such as grid or random search, evolutionary algorithms, Bayesian optimization, Hyperband and racing. It gives practical recommendations regarding important choices to be made when conducting HPO, including the HPO algorithms themselves, performance evaluation, how to combine HPO with ML pipelines, runtime improvements, and parallelization. This work is accompanied by an appendix that contains information on specific software packages in R and Python, as well as information and recommended hyperparameter search spaces for specific learning algorithms. We also provide notebooks that demonstrate concepts from this work as supplementary files.

==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{\tilde{r}^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{\tilde{r}^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}


==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}


==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
\newcommand{\HS}{\Phi}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


\newcommand{\alphah}{\hat{\alpha}}													% alpha-hat
\newcommand{\alphav}{\bm{\alpha}}													% vector alpha (bold)
\newcommand{\alphavh}{\hat{\bm{\alpha}}}													% vector alpha-hat



\newcommand{\phix}{\phi(\xv)}          												% \phi(x)
\newcommand{\phixt}{\phi(\tilde \xv)}        										% \phi(x-tilde)



==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}


==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  

